Bi-Arc Digraphs and Conservative Polymorphisms

In this paper we study the class of bi-arc digraphs, important from two seemingly unrelated perspectives. On the one hand, they are precisely the digraphs that admit certain polymorphisms of interest in the study of constraint satisfaction problems; on the other hand, they are a very broad generalization of interval graphs. Bi-arc digraphs is the class of digraphs that admit conservative semilattice polymorphisms. There is much interest in understanding structures that admit particular types of polymorphisms, and especially in their recognition algorithms. (Such problems are referred to as metaproblems.) Surprisingly, the class of bi-arc digraphs also describes the class of digraphs that admit certain other kinds of conservative polymorphisms. Thus solving the recognition problem for bi-arc digraphs solves the metaproblem for digraphs for several types of conservative polymorphisms. The complexity of the recognition problem for digraphs with conservative semilattice polymorphisms was an open problem, while it was known to be NP-complete for certain more complex relational structures. We complement our result by providing a complete dichotomy classification of which general relational structures have polynomial or NP-complete recognition problems for the existence of conservative semilattice polymorphisms. Bi-arc digraphs also generalizes the class of interval graphs; in fact it reduces to the class of interval graphs for symmetric and reflexive digraphs. It is much broader than interval graphs and includes other generalizations of interval graphs such as co-threshold tolerance graphs and adjusted interval digraphs. Yet, it is still a reasonable extension of interval graphs, in the sense that it keeps much of the appeal of interval graphs. Our main result is a forbidden obstruction characterization of, and a polynomial recognition for, the class of bi-arc digraphs.

==> Hypergraphs.tex <==
\section{Higher arity}\label{hypergraph}

Let $A$ denote a finite set (domain also called scope). By a $k$-ary relation $R$ on a domain $A$ we mean a subset of the $k$-th cartesian power $A^k$; $k$ is said to be the \emph{arity}
of the relation. A constraint language $\Gamma$ over $A$ is a set of relations over $A$. A constraint language is finite if it contains finitely many relations. 
\begin{definition}
A constraint over a constraint language $\Gamma$ is an expression of the form $R(x_1,...,x_k)$ where $R$ is a relation of arity $k$ contained in $\Gamma$, and the $x_i$ are variables. A constraint is satisfied by a mapping $\phi$ defined on the $x_i$ if $(\phi(x_1),\dots , \phi(x_k)) \in R$.
\end{definition}
\begin{definition}
An instance  $(V ; A; {C_1 ,\dots , C_m })$ of a constraint satisfaction problem consists of
\begin{itemize}
    \item a finite set of variables, $V = \{x_1,\dots,x_n\}$;
    \item a finite domain of values, $A$;
    \item a finite set of constraints, $\{C_1,\dots , C_m\}$; where each constraint $C_l, l \in [m]$, is a pair $((x_{i_1},\dots,$ $x_{i_{k_l}}),R_l)$, with
    \begin{itemize}
        \item $(v_{i_1} , \dots , v_{i_{k_l}})$ is a tuple of variables of length $k_l$, called the constraint scope, and
        \item $R_l$ is a $k_l$-ary relation on $A$, called the constraint relation.
    \end{itemize}
\end{itemize}
\end{definition}
A solution to a CSP instance is a mapping $\phi : V \to A$ such that for each constraint $C_l, l \in [m]$, we have that $(\phi(x_{i_1}),\dots,\phi(x_{k_l})) \in R_l$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%commented by Akbar
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Let $(V,C,A,T)$ be an instance of the CSP($T$) problem. Here $V$ is the set of variables $x_1,\dots, x_n$, and $C$ is a set of constraints and $T$ is the target relation on the scope set $A$. Each constraint $C_i$ is of form $(x_{i_1},x_{i_2},\dots,x_{i_k}) \in V^k$  (a tuple from the domain) and a 
%list $$\{(a^1_1,a^1_2,\dots,a^1_k), (a^2_1,a^2_2,\dots,a^k_k),\dots,  (a^r_1,a^r_2,\dots,a^r_k)\}$$ of possible images (scope)  from $A^k$.  The goal is to find a mapping from $V$ to $A$ in order to satisfy all the constraints at the same time. In other words, the goal is to find a homomorphism from $V$ to $A$ where the image of every tuple from the domain lies in its scope. 

\begin{definition}[Signature]
    %Let $(V ; A; {C_1 ,\dots , C_m })$ be an instance of a CSP with relation $R$. 
    For every pair of tuples $t_1,t_2\in R$ we associate a signature
    $$S_{t_1,t_2}=\{(i,j,k) | 
    \text{ k-th element of $A$ appears in i-th coordinate of $t_1$ and in  j-th coordinate of $t_2$ } \}.$$
  
   %\anote{what is $V$ (or $A$)?}
     
    %where $S_i,S_j \subseteq \{1,2,\dots,k\}$, and $S_i$ is the coordinates set of the variables of $C_i$, appearing in $C_j$, and $S_j$ is the coordinate set of the variables of $C_j$ appearing in $C_i$. Here $k$ is the maximum of arity of %$t_1,t_2$. 
\end{definition} 




We construct a graph $G$ as follows. The vertices of $G$ are the pairs $(t_1,t_2)$ where $t_i$, $i=1,2$ are tuples of $R$  with the same arity. 
We put an edge $xy$ in $G$ between $x=(t_1,t_2)$ and $y=(t'_1,t'_2)$ if the signatures of $(t_1,t'_1),(t_2,t'_2)$ are the same. 

The list of vertex $x=(t_1,t_2) \in G$, $L(x)$, is the set of all tuples $t_3 \in R$ with the same arity as $t_1,t_2$, and satisfying the following condition:

\begin{itemize} 
\item  The $i$-th coordinate of $t_3$ is either the same as $i$-th coordinate of $t_1$ or the $i$-th coordinate of $t_2$.
%\anote{do you mean if there exists a coordinate $i$?}
\end{itemize}

 The vertices of $H$ is the union of all the vertices in lists of the vertices in $G$  
%\anote{what is the vertex set of H? what is the edge set of H?} 
Note that the size of $H$ is $|R|2^k$, where $|R|$ is the number of tuples in $R$. 
%\Rnote{ $T=R$, $\hat{t}$ is the corresponding vertex to tuple $t$} 
We put an edge (in $H$) between $\hat{t} \in L(x)$ and $\hat{t'} \in L(y)$ (in $H$ ) if $(\hat{t},\hat{t'}),(t_1,t'_1)$ have the same signature.

%\anote{what is $(t_1,t'_1)$? what about %$(t_2,t'_2)$?}. 

\begin{definition}
Let $G,H,L$ 
%\anote{are these the same as above?} 
be an instance of the list homomorphism. $G$ is the input (di)-graph and $H$ is the target (di)-graph and $L$ is the lists; subset of $V(H)$. 
Let $GH=G \times_L H^2$ be a graph with vertex set $\{(x,a,b)| x \in V(G), a,b \in L(x)\}$.  We say $GH$ admits a semmi-lattice if  there exists a homomorphism $f : GH \rightarrow H$ with the following properties:

\begin{itemize}
\item $f(x,a,b) \in L(x)$,
\item $f(x,a,b)=f(x,b,a) \in \{a,b\}$,
\item  $f(x,a,f(x,b,c))=f(x,f(x,a,b),c)$,
\item $f(x,a,b)f(x',a',b') \in E(H)$ when $xx' \in E(G)$, $aa',bb' \in E(H)$.
\end{itemize}
\end{definition}

\begin{proposition}
$R$ has a conservative semmi-lattice polymorphism iff $GH$ admits a min ordering.
\end{proposition}

In order to decide whether $GH$ admits a semmi-lattice we do the following. 

Construct an auxiliary digraph $D^+$ as follows. 
$V(D^+)=V(GH)$. The arc set of $D^+$ is the set of $\{ (x,a,b)(x',b',c') | xx' \in E(G), aa',bb' \in E(H), ab' \not\in E(H)\}$.

We say $D^+$ has a strong circuit if $(x,a_0,a_1),(x,a_1,a_2),\dots,(x,a_{n-1},a_n),(x,a_n,a_0)$ belong to the same strong component of $D^+$. Now following Theorem \ref{main-k} we can deploy the same algorithm to decide whether $D^+$ has a semmi-lattice. 

